Frugal Actor-Critic: Sample Efficient Off-Policy Deep Reinforcement Learning Using Unique Experiences

Efficient utilization of the replay buffer plays a significant role in the off-policy actor-critic reinforcement learning (RL) algorithms used for model-free control policy synthesis for complex dynamical systems. We propose a method for achieving sample efficiency, which focuses on selecting unique samples and adding them to the replay buffer during the exploration with the goal of reducing the buffer size and maintaining the independent and identically distributed (IID) nature of the samples. Our method is based on selecting an important subset of the set of state variables from the experiences encountered during the initial phase of random exploration, partitioning the state space into a set of abstract states based on the selected important state variables, and finally selecting the experiences with unique state-reward combination by using a kernel density estimator. We formally prove that the off-policy actor-critic algorithm incorporating the proposed method for unique experience accumulation converges faster than the vanilla off-policy actor-critic algorithm. Furthermore, we evaluate our method by comparing it with two state-of-the-art actor-critic RL algorithms on several continuous control benchmarks available in the Gym environment. Experimental results demonstrate that our method achieves a significant reduction in the size of the replay buffer for all the benchmarks while achieving either faster convergent or better reward accumulation compared to the baseline algorithms.

==> introduction.tex <==
\section{Introduction}
Occam’s razor states that plurality must never be posited without necessity. In the context of off-policy controller synthesis, it can be described as, if a controller can be synthesized from multiple set of samples, one with smaller set %\is{simpler in which sense?}\ns{fixed} 
is to be preferred.
This means discarding or shaving away the redundant samples from the given set of samples and still getting the same result.

\paragraph{General Introduction}
In \cite{Mnih2015}, the authors demonstrated the power of DQN in solving various Atari games using replay buffer of size $10^6$. Similarly, the same size of $10^6$ was used in ~\cite{Lillicrap15} to solve various Mujoco-based tasks. This became a default size for the community as evident in later works of ~\cite{Andrychowicz17},~\cite{tassa18},~\cite{stable-baselines3} etc.

In this work we demonstrate that not all samples are needed to learn the controller. In fact, we may synthesize a controller with samples as few as $90\%$ than the state-of-the-art off-policy actor-critic algorithms. This means that our replay buffer size can be reduced significantly.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{drb.pdf}
%     \caption{Default Replay buffer}
%     \label{fig:drb}
% \end{figure}



\paragraph{Correlation is a problem}
Typically, an RL agent encounters sequences of highly correlated states and learning from these correlated data points is not desirable~\cite{Lillicrap15}. This is because Controller synthesis %\is{provide full form}\ns{done} 
algorithms suffer from high estimation variance when data samples are dependent, leading to
slower and potentially less stable learning~\cite{LeCun12,Bengio12}. Thus, we need a method that de-correlates the samples stored in RB, so as to improve data efficiency and reduce sample complexity.

Due to correlation between samples, the independent and identically distributed (i.i.d) assumption is violated, which is critical for Stochastic Gradient Descent (SGD) optimization. This leads to very high variance in gradients~\cite{Needell14,Zhao15}, which means that our training batch contains very similar examples, each of these  pushing our network in the same direction. However, this may be totally the wrong direction in the global sense, as all those examples could be from one single lucky or unlucky episode. 
This is solved by storing a large amount of previous states in the replay buffer and sampling mini-batches from this buffer. If the buffer is large enough, the random sample from it is much better representation of the states distribution at large. 

Also, having a replay buffer with only fairly distinct samples ensures the i.i.d. assumption. The i.i.d. sampling is important to ensure that the stochastic gradient is an unbiased estimate of the full gradient. 


\paragraph{Smaller replay buffer is important}
As the systems becomes more complex, the states and action spaces become high dimensional. This leads to larger memory size to store transitions in replay buffer. For example, the default size of replay buffer for the Ant and Humanoid is $\texttt{1.7GB}$ and  
$\texttt{5.7GB}$ respectively.
This problem is caused mainly because the current algorithms simply add all the transitions encountered so far directly into the replay buffer. %%\st{Using FAC} \is{Introduce it before}\ns{fixed} 
This can be addressed by adding only the required transitions into the replay buffer.


The main challenge in reducing replay buffer size is to identify the set of samples that are enough to learn a controller of similar performance. 
This is hard for continuous control problems with continuous state and
action spaces. This is because of very rare chance that two states or action would be the same. This problem becomes even harder for high-dimensional spaces. Moreover, the algorithm should be fast enough to not incur any significant additional overhead so that insertion and sampling from replay buffer remains computationally feasible.  

The work~\cite{zhang17} discusses that having large replay buffer is not necessarily beneficial. In fact, it is sometime detrimental to controller synthesis. There is a trade-off between \textit{data quality} and \textit{data correlation}. In case of smaller replay buffers, only the most recent data is stored but it is often correlated. In case of larger replay buffers, data is \textit{i.i.d.} but also contains a lot of outdated data which might not be very useful for learning. 
Apart from these, smaller replay buffer suffer from \textit{data sufficiency} issue which means not having enough representative samples to synthesize the controller.


However, the reduction in size should not come at the cost of loss in representation, i.e., having sufficient number of samples that can provide a good approximation of the true gradient. This is a challenging problem as identifying similarity of samples is computationally expensive in continuous and high-dimensional domains.


\paragraph{How FAC addresses the concerns}
We propose an algorithm Frugal Actor-Critic (FAC) to address the above issues. The performance of FAC is much better when the exploration is not good, i.e., poor distribution of data samples. Given that the state-of-the-art algorithms like SAC are already quite robust as well as efficient in exploration, there is obviously less scope for improvement. Even then the performance of FAC is better on most benchmarks. It is also worth noting that Deep-RL based controller synthesis are known to have stability issues (due to presence of noise in gradient estimators~\cite{lyle22,Mnih2015}) and hence an exact comparison is not ideal. 
We therefore posit that the performance of two approaches are similar if the average reward accumulated by the controller is in close range.  However, theoretically, we prove that FAC algorithm is better than general off-policy actor-critic algorithms in storing i.i.d. samples in replay buffer as well as in convergence.
To the best of our knowledge, no prior algorithm have been proposed to control the storage of samples into the replay buffer in this setting.


Note that naively discarding samples whose state is similar to those present in replay buffer might lead to degradation in learning (since samples with similar states can have different rewards) %\is{Why?}\ns{done} 
and hence synthesis of sub-optimal controllers. Since, the learning depends on reward maximization, the controller needs the knowledge of different rewards achieved for a given state (by taking different actions). Hence, we needs to keep samples corresponding to different rewards for a given state.     


% Reduction in samples - > overparameterization > leads to simpler policy. This is evident from low control cost.
% \url{https://openreview.net/pdf?id=HJli2hNKDH}
% TD3- Deterministic
% SAC - Stochastic

